EdgeNets:Edge Varying Graph Neural Networks

Driven by the outstanding performance of neural networks in the structured Euclidean domain, recent years have seen a surge of interest in developing neural networks for graphs and data supported on graphs. The graph is leveraged at each layer of the neural network as a parameterization to capture detail at the node level with a reduced number of parameters and computational complexity. Following this rationale, this paper puts forth a general framework that unifies state-of-the-art graph neural networks (GNNs) through the concept of EdgeNet. An EdgeNet is a GNN architecture that allows different nodes to use different parameters to weigh the information of different neighbors. By extrapolating this strategy to more iterations between neighboring nodes, the EdgeNet learns edge- and neighbor-dependent weights to capture local detail. This is a general linear and local operation that a node can perform and encompasses under one formulation all existing graph convolutional neural networks (GCNNs) as well as graph attention networks (GATs). In writing different GNN architectures with a common language, EdgeNets highlight specific architecture advantages and limitations, while providing guidelines to improve their capacity without compromising their local implementation. An interesting conclusion is the unification of GCNNs and GATs -- approaches that have been so far perceived as separate. In particular, we show that GATs are GCNNs on a graph that is learned from the features. This particularization opens the doors to develop alternative attention mechanisms for improving discriminatory power.

==> sec_mult.tex <==
% !TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%TABLE%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}
\centering
\caption{Summary of the different GNN architectures and their respective characteristics. The parameters and the complexity is considered per layer. Legend: $N$- number nodes; $M$- number of edges; $F$- maximum number of features; $K$- the recursion order; $b$- dimension of the Kernel in \eqref{eq:paramSpec}; $\bbB_{\bbV,\ccalI}$- basis matrix in \eqref{eq.basMat}; $\ccalB$- the set of priviledged nodes in \eqref{eq.nvGCNN} and \eqref{eq.nvGCNN1}; $N_{\ccalB}$- maximum number of neighbors for the nodes in $\ccalB$; $P$- parallel J-ARMANet branches; $t$- Jacobi iterations; $R$- parallel attention branches; $M_\text{tot}$- total number of edges in the multi-edge feature networks; $E$- maximum number of edge features for the multi-edge category. $^*$Self-loops are not considered. $^{**}$The eigendecomposition cost $\ccalO(N^3)$ is computed only once for all layers.}
\begin{tabular}{| c | c | c | c | }
  \hline			
  Architecture & Expression & Parameters$^*$ & Complexity$^{*, **}$\\
  \hline \hline
Fully connected & n/a & $N^2F^2$  & $\ccalO(N^2F^2)$\\
\textbf{Edge variant} & Eq.~\eqref{eqn_gnn_filters} & $KF^2M$  & $\ccalO(KF^2M)$\\
\hline \hline
GCNN \cite{defferrard2016convolutional, kipf2016semi,du2017topology, gama2018convolutional} & Eq. \eqref{eq:gcnn} & $(K+1)F^2$ & $\ccalO(KF^2M)$\\
Node varying \cite{gama2018convolutionalNV} & Eq. \eqref{eq.nvGCNN} &$(K+1)|\ccalB|F^2$ & $\ccalO(KF^2M)$\\
\textbf{Node dependent edge varying}& Eq. \eqref{eq.nvGCNN1} & $\big((K+1) + |\ccalB| + KN_\ccalB	\big)F^2$ & $\ccalO(KF^2M))$\\
\textbf{Spec. edge varying GCNN} & Eq.~\eqref{eq.EV_respfinProp} & $K\rank(\bbB_{\bbV,\ccalI})F^2$ & $\ccalO(KF^2M)$ + $\ccalO(N^3)$\\
Spec. Kernel GCNN \cite{bruna2013spectral} & Eq.~\eqref{eq.EV_respfinProp} for $K = 1$ & $bF^2$ & $\ccalO(N^2F^2)$ + $\ccalO(N^3)$\\
\textbf{J-ARMANet} & Eq. \eqref{eq:propClaim} & $(2P + K^\prime + 3)F^2$ & $\ccalO\big(F^2M\big((P+1)(t+1) + K^\prime\big) + NF^2(P+1)\big)$\\
\hline \hline
\textbf{GCAT} & Eq. \eqref{eq:polyGatfg} & $R(F^2 + 2F + K+1)$ & $\ccalO\big(R(NF^2+ KFM)\big)$\\
GAT \cite{velickovic2017graph} & Eq. \eqref{eq:polyGatfg} for $K = 1$ & $R(F^2 + 2F)$ & $\ccalO\big(R(NF^2+FM)\big)$\\
\textbf{Edge varying GAT} & Eq. \eqref{eq:evGAT} & $R\big((K+1)F^2 + 2KF\big)$  &$\ccalO(RKF(NF + M))$\\
\textbf{W-GCAT} & Eq. \eqref{eq.wGCAT} & $R(F^2 + 2F + K+1)$ & $\ccalO\big(R(NF^2+ KFM)\big)$\\
\textbf{Hybrid GCAT} & Eq. \eqref{eq.HybGCAT} & $R(F^2 + 2(F + K+1))$ & $\ccalO\big(R(NF^2+ KFM)\big)$\\
\hline \hline
\textbf{Multi-edge varying} & Eq. \eqref{eq:EVhlFEd} & $KF^2EM_{\text{tot}}$  & $\ccalO(KF^2EM)$\\
\textbf{Multi-edge GCNN} & Eq. \eqref{eq.multEgpol} &$(K+1)EF^2$ & $\ccalO(KF^2EM)$\\
\textbf{Multi-edge convolutional GAT} & Eq. \eqref{eq:multiGAT} &$RE(F^2 + 2F + K + 1)$ & $\ccalO(RE(NF^2+KFM))$\\
\hline
\end{tabular}
\label{tab:sum}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The former sections considered a graph that has a single feature per edge (i.e., the edge weight). Nevertheless, when the graph connectivity is characterized by multiple edge features \cite{kawahara2017brainnetcnn,ioannidis2019recurrent}, this aspect can be exploited to enhance the learning capabilities of the network. 

Let then $\ccalG = (\ccalV, \ccalE)$ be a graph of $N$ nodes but with an edge set $\ccalE \subseteq \ccalV\times\ccalV$ that has a total of $M_\text{tot}$ edges and a weight function $\ccalW : \ccalV\times\ccalV \to \reals^{E}$. That is, over each edge there is a vector of $E$ features. This multi-edge graph consists of the union of $E$ subgraphs $\ccalG_e = (\ccalV, \ccalE_e)$ each having the same nodes but a different edge set $\ccalE_e$ and weights function $\ccalW_e : \ccalV\times\ccalV \to \reals$. Denote by $M_e$ the number of edges of subgraph $\ccalG_e$ such that $M_\text{tot} = M_1 + \ldots + M_{E}$. Each of these subgraphs is now characterized by its own shift operator matrix $\bbS_e$. We can therefore extend the proposed framework to operate on each subgraph and aggregate the higher level features in building the layer output.

\textbf{Edge varying.} Let $\bbx_g$ be the $g$th layer input feature residing on the nodes of the graph $\ccalG$ with $E_l$ edge features. The processing of these features is now carried by $E_l$ filter banks of $F_l \times F_{l-1}$ filters of the form \eqref{eq:evFG}, where the $e$th filter bank  operates on the subgraph $\ccalG_e$ for $e = 1, \ldots, E_l$. The filter outputs are aggregated across all input features and subgraphs to obtain produce the $f$th higher level feature
%
\begin{align}\label{eq:EVhlFEd}
\begin{split}
\bbu_f = \sum_{e = 1}^{E_l}\sum_{g = 1}^{F_{l-1}}\sum_{k=1}^{K}\bbPhi_{efg}^{(k:1)}\bbx_g\quad \text{for}~f = 1, \ldots, F_l
\end{split}
\end{align}
%
where the edge varying parameter matrix $\bbPhi_{efg}^{l(k)}$ shares the support with $\bbS_e + \bbI_N$. This implementation allows to build the output features as an edge weight aggregation of the input features over the different subgraphs followed by a pointwise nonlinearity.

Set $E = \max_l E_l$, $M = \max_{l,e} M_e^l$, and recall that $F = \max_{l}F_l$. Then, the total number of parameters per layer of the implementation in \eqref{eq:EVhlFEd} is at most $KF^2(M_\text{tot}+NE)$. Likewise, the order of complexity per layer is $\ccalO(KF^2E(M+N))$. %This recursion represents the edge varying extension of edge varying filter to the case of multi-edge features.

\textbf{GCNN.} Similar to \eqref{eq:EVhlFEd}, a multi-edge graph convolutional layer can be considered as the extension of the polynomial filter in \eqref{eq:gcnn} to the multiple-edge feature context. The $f$th higher level feature of this implementation is
%
\begin{equation}\label{eq.multEgpol}
\bbu_f = \sum_{e = 1}^{E_l}\sum_{g = 1}^{F_{l-1}}\sum_{k = 0}^K\phi_{efg}^{(k)}\bbS_e^k\bbx_g \quad \text{for}~f = 1, \ldots, F_l.
\end{equation}
%
That is, it consists of a polynomial in $\bbS_e$ of order $K$ for each graph $\ccalG_e$. This parameterization has $(K+1)EF^2$ coefficients and an order of complexity that is similar to \eqref{eq:EVhlFEd}. Following the derivations in Section~\ref{sec:gcnn}, the other GCNN techniques can be readily extended to the multi-edge scenario.

\textbf{GCAT.} In a similar way, we can extend the convolutional GAT to the multi-edge case. Shortly, let $\bbW_e \in \reals^{F_l\times F_{l-1}}$ be the transform matrix w.r.t. the graph $\ccalG_e$ and $\bba_e \in \reals^{2F_l}$ the corresponding attention coefficient vector. The higher level features of the GCAT filter are
%
\begin{equation}\label{eq:multiGAT}
\bbU = \sum_{e = 1}^{E_l}\sum_{k = 0}^K\phi_{ek}\bbPhi_e^k\bbX\bbW_e^\transp
\end{equation}
%
where $\bbPhi_e$ is the GAT-learned shift operator matrix w.r.t. the graph $\ccalG_e$. The multi-edge GAT is basically parameterizing \eqref{eq:EVhlFEd} with a different attention mechanism for each subgraph $\ccalG_e$. This parameterization yields a total number of parameters per layer of at most $RE(F^2 + 2F + K + 1)$ and a computational complexity of order $\ccalO(RE(NF^2+KFM))$. As for the multi-edge GCNN, the extensions and discussion in Section~\ref{sec:gat} can be readily generalized to the multi-edge scenario. 

Table~\ref{tab:sum} concludes the theoretical part of the paper with a summary of the different architectures and their properties.





